Online Buy-at-Bulk Network Design

We present the first non-trivial online algorithms for the non-uniform, multicommodity buy-at-bulk (MC-BB) network design problem in undirected and directed graphs. Our competitive ratios qualitatively match the best known approximation factors for the corresponding offline problems. The main engine for our results is an online reduction theorem of MC-BB problems to their single-sink (SS-BB) counterparts. We use the concept of junction-tree solutions (Chekuri et al., FOCS 2006) that play an important role in solving the offline versions of the problem via a greedy subroutine -- an inherently offline procedure. Our main technical contribution is in designing an online algorithm using only the existence of good junction-trees to reduce an MC-BB instance to multiple SS-BB sub-instances. Along the way, we also give the first non-trivial online node-weighted/directed single-sink buy-at-bulk algorithms. In addition to the new results, our generic reduction also yields new proofs of recent results for the online node-weighted Steiner forest and online group Steiner forest problems.

==> prelims.tex <==
\section{Reduction to Layered Instances}
In this section, we show an extension of Zelikovsky's `height reduction lemma' for the buy-at-bulk problem 
(i.e., Zelikovsky's original Lemma only cared about one metric, whereas we need to work with a cost metric and a length metric). 
We mention it up front as it will be used in a couple of different places, and also because it could be of interest in general.

\begin{theorem} \label{thm:layering}
Given a directed graph $G = (V,E)$ with edge costs $c_e$ and lengths $\ell_e$, for all $h>0$, we can efficiently find a {\em up-ward directed, layered} directed graph $G^\upp_h$ on $(h+1)$ levels and edges (with new costs and lengths) only between successive levels going from bottom to top, such that each layer has $n$ vertices corresponding to the vertices of $G$, and, for any set of terminals $X$ and any root vertex $r$,
\begin{OneLiners}
\item[(i)] the optimal objective value of the {\em single-sink}  buy-at-bulk problem to connect $X$ (at level $h$) with $r$ (at level $0$) on the graph $G^{\upp}_h$ is at most $O(h k^{\frac1h}) \phi$, where $\phi$ is the objective value of an optimal solution of the same instance on the original graph $G$,
\item[(ii)] given a integral/fractional solution  of objective value $\phi$ for the single-sink buy-at-bulk problem to connect $X$ with $r$ on the graph $G^{\upp}_h$, we can efficiently recover an integral/fractional solution of objective value  at most $\phi$ for the problem on the original graph $G$.
%\item[(iii)] the integrality gap of natural LP for the single-sink buy-at-bulk problem to connect $X$ with $r$ in $G_h$ is at most the integrality gap in $G$.
\end{OneLiners}
Likewise, we can obtain a down-ward directed, layered graph $G^{\downn}_h$ on $(h+1)$-levels with edges going from top to bottom, with the same properties as above except for single-source instances instead.
\end{theorem}

\begin{proof}
We prove the up-ward case; the down-ward follows analogously. We also lose the supersctipt $^\upp$.
For this reduction, we will adapt the notion of layered expansion of a graph,
which has been in the folklore for many years and has been used recently by several papers
(see, e.g.,\cite{ChekuriEGS11, NaorPS11}). The $h$-level {\em layered expansion} of $G$ is a layered DAG $G_h$
of $h+1$ levels (we index the level $0, 1, \ldots, h$) defined as follows:
\begin{OneLiners}
	\item[(i)] The vertices in levels $i$, for $0\leq i\leq h$ are copies of the vertices of $G$: we let $v_i$ to denote the copy of vertex $v \in V$ at level $i$.
    \item[(ii)] There is a directed edge from every vertex in level $i$ to every vertex in level $i-1$ (for $1 \leq i \leq h$). The fixed cost of an edge $(u_i, v_{i-1})$ is
	given by that of the shortest directed path $P^i_{uv}$ from $u_i$ to $v_{i-1}$ in $G$ according to the metric $c_e + k^{1 - i/h} \ell_e$. The length of this edge is set to be the length of the path $P^i_{uv}$ in the $\ell$ metric.
\end{OneLiners}

We now relate the optimal objective value for the two instances. One of the directions of the reduction is straightforward.

\begin{lemma}
\label{lma:layered2directed}
For any root $r$ and any set of terminals $X$, if there is a feasible integral/fractional solution of objective/LP value $\phi$ for the single-sink buy-at-bulk problem connecting $X$ to $r$ on the $h$-level layered expansion $G_h$, then there is a feasible integral/fractional solution of objective/LP at most $\phi$ for the same problem in $G$. %Likewise, the optimal LP solution for this instance on $G_h$ has cost at least that of the optimal fractional solution on $G$.
\end{lemma}
\begin{proof}
	Note that for every edge in $G_h$, there is a corresponding path
	in $G$ with the property that the sum of edge costs and lengths on the
	path is at most the cost and length of the edge in $G$. Therefore,
	replacing the edges in the solution for the layered graph by the corresponding
	paths in $G$ yields a feasible solution in $G$
	without increasing the overall cost and length. Notice that the same ``embedding'' of edges in $G_h$ to paths in $G$ can be applied to the  fractional solution on $G_h$ as well. This shows property (ii) of the theorem statement.
\end{proof}

The more interesting direction is to show that the optimal objective value  on the layered graph $G_h$ can be bounded in terms of the optimal objective value on the original graph $G$. To show this, we will re-purpose the so-called ``height reduction'' lemma of Helvig, Robins, and Zelikovsky~\cite{HelvigRZ01}. We restate the lemma in a form that will be useful for us.
\comment{Don't we need to provide a proof of the lemma below? I couldn't find the statement in Helvig et al. -- deepc}
\begin{lemma}
	\label{lma:height-reduction}
 	For any in-tree $T$ defined on the edges of $G$ that is rooted at $r$
 	and contains all the terminals in $X$, and for any integer $h \geq 1$, there is an
 	in-tree $T'$ (on the same vertices as $G$ but over a different edge set) that is also rooted at $r$ and contains
 	all the terminals, and has the following properties:
 	\begin{OneLiners}
 		\item[(i)] $T'$ contains $h+1$ levels of vertices, i.e., has height $h$.
 		\item[(ii)] $T'$ is an $k^{1/h}$-ary tree, i.e., each non-leaf vertex has
 		$k^{1/h}$ children.
 		\item[(iii)] Each edge $e' = (u',v')$ in tree $T'$ corresponds to the unique directed path $p_{e'}$
 		in $T$ from $u'$ to $v'$. Moreover, the number of terminals in the subtree
 		of $T$ rooted at $u'$ is exactly $k^{1-i/h}$, where $e'$ is an edge between
 		levels $i-1$ and $i$ of $T$.
 		\item[(iv)] Each edge in $T$ is in at most $2h k^{1/h}$ such paths $p_{e'}$
 		for edges $e'\in T'$.
 	\end{OneLiners}
\end{lemma}

Now, for an edge $e' \in T'$, suppose we define its cost to be the cost of the path $p_{e'}$, and its length to be the length of the path $p_{e'}$. Then, it is easy to see that the overall cost $\phi_{T'}$ of tree $T'$ is $O(h k^{1/h})$ times that of tree $T$: this is due to the following implications of the above lemma: (a) the total (buying) cost of all edges in $T'$ is at most $2h k^{1/h}$ times that of $T$ since each edge is reused at most $2h k^{1/h}$ times, and (b) for any terminal $x \in X$, the edges on its path to the root in $T'$ correspond to disjoint sub-paths in the unique path between $x$ and $r$ in $T$, and hence the total length cost in $T'$ is at most that in $T$.

Now, using this lemma, we can now complete the reduction by ``embedding'' the tree $T'$ in the layered graph $G_h$.

\begin{lemma}
\label{lma:directed2layered}
	If there is a feasible solution of overall cost $\phi$ for the single-sink buy-at-bulk problem on $G$, then there is a feasible solution of overall cost
	$O(h k^{1/h} \phi)$ for the same problem on the $h$-level
	layered extension $G_h$.
\end{lemma}
\begin{proof}
	Let $T$ be the union of the paths in the optimum solution on the graph $G$. It's easy to see that $T$ is a directed in-tree. 
First, we use Lemma~\ref{lma:height-reduction} to transform
	$T$ to tree $T'$ of height $h$. As noted earlier, the overall cost $\phi_{T'}$ of
	$T'$ is $O(h k^{1/h} \phi)$. Now, we construct a feasible tree $T_h$ in
	$G_h$ using this solution $T'$ as follows: consider each edge $(u,v)$ in $T'$ where $u$ is at level $i$ and $v$ is at level $(i-1)$. Then, include the edge $(u_i, v_{i-1})$ in $T_h$.
    Clearly, since $T'$ connects all the terminals to the root, so does $T_h$. Moreover, notice that there is a 1-to-1 mapping between edges in $T'$ and edges in $T_h$.

To bound the objective value of
	the subtree, we bound the objective value for each  edge of the subtree in
	$G_h$ to its corresponding mapped edge in $T'$.
    First, note that the overall contribution of to an edge $e' = (u',v')$ between layers $i$ and
	$i+1$ towards $\phi_{T'}$ is equal to the sum of costs and $k^{1-i/h}$ times the
	lengths of the edges on the associated path $p_{e'}$ from $u'$ to $v'$.
    This is because, by property (iii) of~\Cref{lma:height-reduction}, the number of demands in the subtree rooted at $u'$ is exactly $k^{1 - i/h}$ and all of them traverse this edge to reach $r$.
    Next, we note that the cost (as we have defined) of the edge $(u'_i, v'_{i+1})$ between layers $i$ and
	$i+1$ in $T_h$ is equal to the \emph{shortest directed path} from
	$u'$ to $v'$ in $G$ according to the metric $c_e + k^{1 - i/h} \ell_e$. Since we chose the shortest path, we get that the buying cost of edge $(u'_i, v'_{i+1}) \in T_h$ is at most the contribution of $(u',v')$ towards $\phi_{T'}$. Moreover, the total length cost is at most $k^{1-i/h}$ times the length of the shortest path, which is at most the fixed cost of $(u'_i, v'_{i+1}) \in T_h$ (again, this uses the fact that there are exactly $k^{1-i/h}$ terminals which route through this edge in $T_h$ also).
	It therefore follows that the overall
	cost of the solution that we have inductively constructed in $G_h$
	is at most twice the overall cost of $T'$, which is at most $O(h k^{1/h}) \phi$.
\end{proof}

~\Cref{lma:layered2directed,lma:directed2layered} then complete the proof of~\Cref{thm:layering}.
\end{proof}

